Analytic calculation of two-loop QCD corrections to b\to s\ell^+\ell^- in the high q^2 region

We present our results for the NNLL virtual corrections to the matrix elements of the operators O_1 and O_2 for the inclusive process b\to s\ell^+\ell^- in the kinematical region q^2>4m_c^2, where q^2 is the invariant mass squared of the lepton-pair. This is the first analytic two-loop calculation of these matrix elements in the high q^2 region. We give the matrix elements as an expansion in m_c/m_b and keep the full analytic dependence on q^2. Making extensive use of differential equation techniques, we fully automatize the expanding of the Feynman integrals in m_c/m_b. In coincidence with an earlier work where the master integrals where calculated numerically (Ghinculov et al.) we find that in the high q^2 region the \alpha_s corrections to the matrix elements <s \ell^+ \ell^-|O_{1,2}|b> calculated in the present paper lead to a decrease of the q^2-spectrum by 10%-15% relative to the NNLL result in which these contributions are put to zero and reduce the renormalization scale uncertainty to ~2%.

==> figs/tab.tex <==
\begin{tabular}{|c|c|r@{\hspace{1ex}}c@{\hspace{1ex}}l|r@{\hspace{1ex}}c@{\hspace{1ex}}l|r@{\hspace{1ex}}c@{\hspace{1ex}}l|r@{\hspace{1ex}}c@{\hspace{1ex}}l|}
\hline
$\sqrt{z}$ & $\hat{s}$ &\multicolumn{3}{c|}{$F_1^{(7)}$} &\multicolumn{3}{c|}{$F_1^{(9)}$} &\multicolumn{3}{c|}{$F_2^{(7)}$} &\multicolumn{3}{c|}{$F_2^{(9)}$}\\
\hline\hline
 & 0.6 & $-0.919$&$-$&0.347$i$ &$7.65$&$-$&26.6$i$ &$5.52$&$+$&2.08$i$ &$15.0$&$+$&10.9$i$ 
\\\cline{2-14}
\raisebox{-2ex}[0ex][-2ex]{0.27} & 0.7 & $-0.905$&$-$&0.402$i$ &$9.07$&$-$&22.7$i$ &$5.43$&$+$&2.41$i$ &$12.0$&$+$&12.6$i$ 
\\\cline{2-14}
 & 0.8 & $-0.888$&$-$&0.449$i$ &$9.78$&$-$&20.0$i$ &$5.33$&$+$&2.69$i$ &$9.44$&$+$&13.3$i$ 
\\\cline{2-14}
 & 0.9 & $-0.869$&$-$&0.488$i$ &$10.2$&$-$&17.9$i$ &$5.21$&$+$&2.93$i$ &$7.35$&$+$&13.6$i$ 
\\\hline\hline
 & 0.6 & $-0.904$&$-$&0.280$i$ &$5.76$&$-$&31.0$i$ &$5.42$&$+$&1.68$i$ &$16.6$&$+$&7.46$i$ 
\\\cline{2-14}
\raisebox{-2ex}[0ex][-2ex]{0.29} & 0.7 & $-0.896$&$-$&0.342$i$ &$8.11$&$-$&26.2$i$ &$5.38$&$+$&2.05$i$ &$13.6$&$+$&10.1$i$ 
\\\cline{2-14}
 & 0.8 & $-0.883$&$-$&0.393$i$ &$9.32$&$-$&22.8$i$ &$5.30$&$+$&2.36$i$ &$11.0$&$+$&11.5$i$ 
\\\cline{2-14}
 & 0.9 & $-0.867$&$-$&0.437$i$ &$9.98$&$-$&20.3$i$ &$5.20$&$+$&2.62$i$ &$8.81$&$+$&12.2$i$ 
\\\hline\hline
 & 0.6 & $-0.879$&$-$&0.208$i$ &$2.65$&$-$&35.9$i$ &$5.28$&$+$&1.25$i$ &$17.9$&$+$&3.06$i$ 
\\\cline{2-14}
\raisebox{-2ex}[0ex][-2ex]{0.31} & 0.7 & $-0.881$&$-$&0.277$i$ &$6.46$&$-$&30.1$i$ &$5.29$&$+$&1.66$i$ &$15.1$&$+$&7.05$i$ 
\\\cline{2-14}
 & 0.8 & $-0.874$&$-$&0.334$i$ &$8.41$&$-$&26.0$i$ &$5.24$&$+$&2.00$i$ &$12.5$&$+$&9.24$i$ 
\\\cline{2-14}
 & 0.9 & $-0.862$&$-$&0.382$i$ &$9.50$&$-$&23.0$i$ &$5.17$&$+$&2.29$i$ &$10.3$&$+$&10.5$i$ 
\\\hline
\end{tabular}

